SMILE: Multimodal Dataset for Understanding Laughter in Video with Language Models

Despite the recent advances of the artificial intelligence, building social intelligence remains a challenge. Among social signals, laughter is one of the distinctive expressions that occurs during social interactions between humans. In this work, we tackle a new challenge for machines to understand the rationale behind laughter in video, Video Laugh Reasoning. We introduce this new task to explain why people laugh in a particular video and a dataset for this task. Our proposed dataset, SMILE, comprises video clips and language descriptions of why people laugh. We propose a baseline by leveraging the reasoning capacity of large language models (LLMs) with textual video representation. Experiments show that our baseline can generate plausible explanations for laughter. We further investigate the scalability of our baseline by probing other video understanding tasks and in-the-wild videos. We release our dataset, code, and model checkpoints on https://github.com/postech-ami/SMILE-Dataset.

==> Figures/supp_AMT_instruction.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{neurips_data_2023/Figures/source/AMT_instruction.pdf}
    \caption{\textbf{Instruction of HITs.} We put the instruction at the top of the interface, describing how the annotators should answer each question.}
    \label{supp_fig:AMT_instruction}
\end{figure}

==> Figures/supp_prompt_gt_candidates.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{Figures/source/prompt_gt_candidates_v2.pdf}
    \caption{\textbf{Prompt for generating laughter reason candidates.} We manually change video types (sitcom or TED) and video title using the meta information of video clips. The query stands for multimodal textual representation $m$ of the video clip. The length of the generated output is also variable, with a maximum of 30 words for sitcoms and 40 words for TED talks, considering each video type's characteristics.}
    \label{supp_fig:prompt_gt_candidates}
\end{figure*}


==> Tables/temp.tex <==
\begin{table*}
  \vspace{2mm}
  
  \centering
  \resizebox{0.75\linewidth}{!}{\begin{tabular}{lcccccc}
    \toprule
    Dataset & Modality & BLEU$_4$ ($\uparrow$) & METEOR ($\uparrow$) & ROUGE$_L$ ($\uparrow$) & BERTScore (F1) ($\uparrow$)\\
    \midrule						
    \multirow{2}{*}{SMILE} & T  & 0.250 & 0.245 & 0.432 & 0.493\\
     & A+V+T  & \textbf{0.270} & \textbf{0.256} & \textbf{0.453} & \textbf{0.496}\\
     \midrule						
    \multirow{2}{*}{SMILE$_{\text{Sitcom}}$} & T  & 0.224 & 0.244 & 0.420 & 0.485\\
     & A+V+T  & \textbf{0.275} & \textbf{0.269} & \textbf{0.469} &\textbf{0.539}\\
     \midrule						
    \multirow{2}{*}{SMILE$_{\text{Ted}}$} & T  & 0.232 & 0.221 & 0.390 & 0.423\\
     & A+V+T  & \textbf{0.234} & \textbf{0.230} & \textbf{0.409} & \textbf{0.462}\\
    \bottomrule
  \end{tabular}}\\
    \caption{\textbf{Evaluation of laugh reasoning using an open-source language model.} We evaluate the laugh reasoning task on LLaMA~\cite{LLAMA} by fine-tuning on \datasetName, and subsets, SMILE$_{\text{Sitcom}}$ and SMILE$_{\text{Ted}}$. Each modality cue in our dataset is denoted as Transcript (T), Audio (A), and Visual (V).}
  \label{sup:results}
\end{table*}


% \begin{table}
%   \caption{Evaluation on laugh reasoning task. In this experiment, we evaluate whether the model can reason about the laughing moment. We use LLaMA~\cite{LLAMA} as the language model for fine-tuning and GPT3~\cite{GPT3} for zero-shot and in-context settings. We further evaluate the models by fine-tuning with the mixed dataset, \ie, mixing with Sitcom and TED videos. Each modality of the attributes in our dataset is denoted as Transcript (T), Audio (A), and Visual (V). FT denotes fine-tuning the model.}
%   \label{sample-table}
%   \centering
%   \resizebox{0.95\linewidth}{!}{\begin{tabular}{lcccccccc}
%     \toprule
%     Dataset & Model & Modality & \multicolumn{4}{c}{Generation} & \multicolumn{1}{c}{Multiple Choice} \\
%     \cmidrule(lr){4-7} \cmidrule(lr){8-8}
%     & & & BLEU$_4$ & METEOR & ROUGE$_L$ & BERTScore (F1) & Accuracy\\
%     \midrule						
%     \multirow{4}{*}{Sitcom}& \multirow{2}{*}{GPT3 (in-context)} & T  & 0.058 & 0.133 & 0.293 & 0.350 & - \\ 						
%      && A+V+T  & 0.059 & 0.140 & 0.303 & 0.353 & 71 (98) \\
%      & \multirow{2}{*}{LLaMA (FT)} & T  & 0.224 & 0.244 & 0.420 & 0.485 & - \\
%      && A+V+T  & \textbf{0.274} & \textbf{0.263} & \textbf{0.471} & \textbf{0.531} & 71 (98) \\
%     \cmidrule{1-8}
%      \multirow{4}{*}{TED}& \multirow{2}{*}{GPT3 (in-context)} & T  & 0.122 & 0.171 & 0.352 & 0.389 & - \\
%      && A+V+T  & 0.173 & 0.204 &0.422  & 0.428 & - \\
%      & \multirow{2}{*}{LLaMA (FT)} & T  & 0.232 & 0.221 & 0.390 & 0.423 & - \\
%      && A+V+T  & \textbf{0.234} & \textbf{0.230} & \textbf{0.409} & \textbf{0.462} & - \\			

%     \bottomrule
%   \end{tabular}}\\
%   \small (a) supervised models comparison\\
%   \vspace{3mm}
%   \resizebox{0.95\linewidth}{!}{\begin{tabular}{lcccccccc}
%     \toprule
%     Dataset & Model & Modality & \multicolumn{4}{c}{Generation} & \multicolumn{1}{c}{Multiple Choice} \\
%     \cmidrule(lr){4-7} \cmidrule(lr){8-8}
%     & & & BLEU$_4$ & METEOR & ROUGE$_L$ & BERTScore (F1) & Accuracy\\
%     \midrule						
%     \multirow{2}{*}{Sitcom}& \multirow{2}{*}{GPT3 (zero-shot)} & T  & 0.046 & 0.110 & 0.247 & 0.306 & - \\
%      && A+V+T  & \textbf{0.052} & \textbf{0.133} & \textbf{0.293} &\textbf{ 0.347 }& - \\
%     \cmidrule{1-8}
%      \multirow{2}{*}{TED}& \multirow{2}{*}{GPT3 (zero-shot)} & T  & 0.096 & 0.141 & 0.297 & 0.342 & - \\
%      && A+V+T  & \textbf{0.142} & \textbf{0.184} & \textbf{0.380 }& \textbf{0.424} & - \\		

%     \bottomrule
%   \end{tabular}}\\
%   \small (b) zero-shot models comparison\\

%   \vspace{3mm}
%   \resizebox{0.95\linewidth}{!}{\begin{tabular}{lcccccccc}
%     \toprule
%     Dataset & Model & Modality & \multicolumn{4}{c}{Generation} & \multicolumn{1}{c}{Multiple Choice} \\
%     \cmidrule(lr){4-7} \cmidrule(lr){8-8}
%     & & & BLEU$_4$ & METEOR & ROUGE$_L$ & BERTScore (F1) & Accuracy\\
%     \midrule						
%     \multirow{2}{*}{Mixed}& \multirow{2}{*}{LLaMA (FT)} & T  & 0.250 & 0.245 & 0.432 & 0.493 & - \\
%      && A+V+T  & \textbf{0.270} & \textbf{0.256} & \textbf{0.453} &\textbf{0.496}& - \\
%     \bottomrule
%   \end{tabular}}\\
%   \small (c) mixed dataset fine-tuning models comparison
  
%   \label{results}
% \end{table}


% \begin{table}
%   \caption{Evaluation on laugh reasoning task. In this experiment, we evaluate whether the model can reason about the laughing moment. We use LLaMA~\cite{LLAMA} as the language model for fine-tuning and GPT3~\cite{GPT3} for zero-shot and in-context settings. Each modality of the attributes in our dataset is denoted as Transcript (T), Audio (A), and Visual (V). FT denotes fine-tuning the model.}
%   \label{sample-table}
%   \centering
%   \resizebox{0.95\linewidth}{!}{\begin{tabular}{lcccccccc}
%     \toprule
%     Dataset & Model & Modality & \multicolumn{4}{c}{Generation} & \multicolumn{1}{c}{Multiple Choice} \\
%     \cmidrule(lr){4-7} \cmidrule(lr){8-8}
%     & & & BLEU$_4$ & METEOR & ROUGE$_L$ & BERTScore (F1) & Accuracy\\
%     \midrule						
%     \multirow{6}{*}{Sitcom}& \multirow{2}{*}{GPT3 (zero-shot)} & T  & 0.046 & 0.110 & 0.247 & 0.306 & - \\
%      && A+V+T  & 0.052 & 0.133 & 0.293 & 0.347 & - \\
%      & \multirow{2}{*}{GPT3 (in-context)} & T  & 0.058 & 0.133 & 0.293 & 0.350 & - \\ 						
%      && A+V+T  & 0.059 & 0.140 & 0.303 & 0.353 & 71 (98) \\
%      & \multirow{2}{*}{LLaMA (FT)} & T  & 0.224 & 0.244 & 0.420 & 0.485 & - \\
%      && A+V+T  & \textbf{0.274} & \textbf{0.263} & \textbf{0.471} & \textbf{0.531} & 71 (98) \\
%     \cmidrule{1-8}
%      \multirow{6}{*}{TED}& \multirow{2}{*}{GPT3 (zero-shot)} & T  & 0.096 & 0.141 & 0.297 & 0.342 & - \\
%      && A+V+T  & 0.142 & 0.184 & 0.380 & 0.424 & - \\
%      & \multirow{2}{*}{GPT3 (in-context)} & T  & 0.122 & 0.171 & 0.352 & 0.389 & - \\
%      && A+V+T  & 0.173 & 0.204 &0.422  & 0.428 & - \\
%      & \multirow{2}{*}{LLaMA (FT)} & T  & 0.232 & 0.221 & 0.390 & 0.423 & - \\
%      && A+V+T  & \textbf{0.234} & \textbf{0.230} & \textbf{0.409} & \textbf{0.462} & - \\			

%     \bottomrule
%   \end{tabular}}
%   \label{results}
% \end{table}

